Simultaneous Deep Transfer Across Domains and Tasks

Recent reports suggest that a generic supervised deep CNN model trained on a large-scale dataset reduces, but does not remove, dataset bias. Fine-tuning deep models in a new domain can require a significant amount of labeled data, which for many applications is simply not available. We propose a new CNN architecture to exploit unlabeled and sparsely labeled target domain data. Our approach simultaneously optimizes for domain invariance to facilitate domain transfer and uses a soft label distribution matching loss to transfer information between tasks. Our proposed adaptation method offers empirical performance which exceeds previously published results on two standard benchmark visual domain adaptation tasks, evaluated across supervised and semi-supervised adaptation settings.

==> tables/crossdataset_supervised.tex <==
\begin{table*}
  \small
  \setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{lcccccc|c}
\toprule
                                 & $I \rightarrow C$  & $C \rightarrow S$  & $C \rightarrow I$ & $I \rightarrow S$ & $S \rightarrow C$ & $S \rightarrow I$ & Average  \\
\midrule
CNN source-only baseline &  \\
CNN target-only baseline \\
CNN source+target baseline \\
\midrule
Ours                             & \textbf{XX.X $\pm$ X.X} & \textbf{XX.X $\pm$ X.X} & \textbf{XX.X $\pm$ X.X}  & \textbf{XX.X $\pm$ X.X}  & \textbf{XX.X $\pm$ X.X}  & \textbf{XX.X $\pm$ X.X}  & \textbf{XX.X} \\
\bottomrule
\end{tabular}

\caption{Multi-class accuracy evaluation on the dense cross-dataset~\cite{crossdata} testbed in the supervised setting.}
\label{table:full-semi}
\end{table*}


==> tables/crossdataset_unsupervised.tex <==
\begin{table*}
  \small
  \setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{lcccccc|c}
\toprule
                                 & $C \rightarrow I$  & $C \rightarrow S$  & $I \rightarrow C$ & $I \rightarrow S$ & $S \rightarrow C$ & $S \rightarrow I$ & Average  \\
\midrule
tommasi's surf baseline \\
CNN source-only baseline \\
CNN source+target baseline \\
\midrule
Ours                             & \textbf{XX.X $\pm$ X.X} & \textbf{XX.X $\pm$ X.X} & \textbf{XX.X $\pm$ X.X}  & \textbf{XX.X $\pm$ X.X}  & \textbf{XX.X $\pm$ X.X}  & \textbf{XX.X $\pm$ X.X}  & \textbf{XX.X} \\
\bottomrule
\end{tabular}

\caption{Multi-class accuracy evaluation on the dense cross-dataset testbed in the unsupervised setting.}
\label{table:full-semi}
\end{table*}


==> tables/office_caltech.tex <==
\begin{table*}
  \scriptsize
  \setlength{\tabcolsep}{2pt}
\centering
\begin{tabular}{lcccccccccccc|c}
\toprule
                               & $A{\rightarrow}W$        & $A{\rightarrow}D$        & $A{\rightarrow}C$        & $W{\rightarrow}A$       & $W{\rightarrow}D$        & $W{\rightarrow}C$        & $D{\rightarrow}A$        & $D{\rightarrow}W$        & $D{\rightarrow}C$       & $C{\rightarrow}A$        & $C{\rightarrow}W$       & $C{\rightarrow}D$        & Average  \\
\midrule                       % A -> W                     A -> D                     A -> C                     W -> A                    W -> D                      W -> C                     D -> A                     D -> W                     D -> C                   C -> A                     C -> W                     C -> D
Source CNN                     &         79.1 $\pm$ 0.5   & \textbf{88.1 $\pm$ 0.5}  &         84.9 $\pm$ 0.1   &         75.3 $\pm$ 0.2  &          98.3 $\pm$ 0.6  &         76.2 $\pm$ 0.1   &         85.8 $\pm$ 0.0   &         98.2 $\pm$ 0.1   &         77.7 $\pm$ 0.1  &         90.9 $\pm$ 0.1   &         78.3 $\pm$ 0.3  &          85.0 $\pm$ 0.6  &         84.8 \\
TTM~\cite{farajidavar2014ttm}  & \textbf{89.8}            &         81.4             &         83.7             & \textbf{88.5}           & \textbf{100.0}           & \textbf{80.4}            & \textbf{90.8}            & \textbf{99.0}            & \textbf{82.9}           &         90.0             & \textbf{86.8}           &  \textbf{89.2}           & \textbf{88.5} \\
\midrule
Ours: dom. confusion           &         83.9 $\pm$ 0.4   & \textbf{88.3 $\pm$ 0.7}  & \textbf{85.5 $\pm$ 0.1}  &         85.1 $\pm$ 0.1  &          98.6 $\pm$ 0.3  & \textbf{80.3 $\pm$ 0.1}  & \textbf{90.9 $\pm$ 0.1}  & \textbf{99.2 $\pm$ 0.0}  &         80.6 $\pm$ 0.1  & \textbf{91.7 $\pm$ 0.1}  &         84.1 $\pm$ 0.3  &          82.4 $\pm$ 0.4  &         87.6 \\
\midrule
\midrule
Target CNN                     &         91.2 $\pm$ 0.9   &         92.9 $\pm$ 1.7   &         77.6 $\pm$ 1.5   &         90.3 $\pm$ 0.5  &          92.9 $\pm$ 1.7  &         77.6 $\pm$ 1.5   &         90.3 $\pm$ 0.5   &         91.2 $\pm$ 0.9   &         77.6 $\pm$ 1.5  &         90.3 $\pm$ 0.5   &         91.2 $\pm$ 0.9  &          92.9 $\pm$ 1.7  &         88.0 \\
Source+Target CNN              & \textbf{94.2 $\pm$ 0.9}  & \textbf{96.3 $\pm$ 1.1}  & \textbf{86.2 $\pm$ 0.4}  & \textbf{92.2 $\pm$ 0.3} &  \textbf{98.3 $\pm$ 0.4} & \textbf{83.5 $\pm$ 0.6}  & \textbf{93.3 $\pm$ 0.3}  & \textbf{99.3 $\pm$ 0.1}  & \textbf{84.6 $\pm$ 0.5} & \textbf{92.6 $\pm$ 0.4}  & \textbf{95.4 $\pm$ 0.4} &  \textbf{95.4 $\pm$ 1.4} & \textbf{92.6} \\
\midrule
Ours: softlabels               &         90.2 $\pm$ 0.7   &         94.3 $\pm$ 0.8   &         85.6 $\pm$ 0.3   &         89.4 $\pm$ 0.7  &  \textbf{98.7 $\pm$ 0.5} &         81.3 $\pm$ 0.3   &         92.3 $\pm$ 0.2   & \textbf{99.4 $\pm$ 0.2}  &         82.7 $\pm$ 0.1  &         91.8 $\pm$ 0.3   &         92.4 $\pm$ 1.1  &          89.8 $\pm$ 1.8  &         90.7 \\
Ours: combined                 & \textbf{94.8 $\pm$ 1.1} &	\textbf{95.5 $\pm$ 1.0} &	\textbf{86.4 $\pm$ 0.3}&	\textbf{92.4 $\pm$ 0.4}&	\textbf{98.6 $\pm$ 0.5}&	\textbf{84.5 $\pm$ 0.5}&	\textbf{93.3 $\pm$ 0.2}&	\textbf{99.6 $\pm$ 0.1}&	83.8 $\pm$ 0.4&	\textbf{92.8 $\pm$ 0.3}&	94.9 $\pm$ 0.4&	93.6 $\pm$ 1.3&	\textbf{92.5} \\
\bottomrule
\end{tabular}

\caption{Multi-class accuracy evaluation on the the \emph{Office-Caltech} dataset. Rows above the double line are from the unsupervised setting, whereas rows below the double line are from the supervised setting.}
\label{table:office-caltech}
\end{table*}


==> tables/office_supervised_allSrc.tex <==
\begin{table*}
  \setlength{\tabcolsep}{4pt}
\centering
                %                 & $A \rightarrow W$  & $D \rightarrow W$  & $W \rightarrow D$  & Average  \\
\begin{tabular}{lcccccc|c c}
\toprule
									&						&						&					&						&						&					& \multicolumn{2}{c}{Averages}\\
									\cline{8-9}
                                 	& $A \rightarrow W$  	& $A \rightarrow D$ 	& $D \rightarrow A$	& $D \rightarrow W$   	& $W \rightarrow A$  	&$W \rightarrow D$  & 3 common shifts		&  all shifts\\
\midrule
DAN~\cite{dan}						&	\textbf{85.6 $\pm$ 0.3}		& --					&		--			&	95.8 $\pm$ 0.2		&	--					  & 96.7 $\pm$ 0.2 & 92.7 & --\\
%Source CNN                 			& 56.5 $\pm$ 0.3 				& 64.6 $\pm$ 0.4  				& 47.6 $\pm$ 0.1    & 92.4 $\pm$ 0.3  & 42.7 $\pm$ 0.1   & 93.6 $\pm$ 0.2  & 66.22 \\
%Target CNN                 			& 80.5 $\pm$ 0.5 				& 81.8 $\pm$ 1.0  				& 59.9 $\pm$ 0.3    & 80.5 $\pm$ 0.5  & 59.9 $\pm$ 0.3   & 81.8 $\pm$ 1.0  & 74.05 \\
%Source+Target CNN           		& \underline{82.5 $\pm$ 0.9} 	& \underline{85.2 $\pm$ 1.1}  	& \underline{65.8 $\pm$ 0.5}  & 93.9 $\pm$ 0.5  & \textbf{65.2 $\pm$ 0.7}  & 96.3 $\pm$ 0.5  & 81.50 \\
\midrule
Ours 	& 83.8 $\pm$ 1.0		&	86.1 $\pm$ 1.0		& 65.0	$\pm$ 0.5	& \textbf{97.0 $\pm$ 0.6}		& 65.0 $\pm$ 0.5		&\textbf{99.4 $\pm$ 0.1}	& \textbf{93.4} & 82.7\\
\bottomrule
\end{tabular}

\caption{Multi-class accuracy evaluation on the standard supervised adaptation
  setting with the \emph{Office} dataset.  We evaluate on all 31 categories
  using the experimental protocol from \cite{dan}. Here, we compare our complete system with a state-of-the-art method DAN~\cite{dan}, which proposed the alterative experimental setting of using all available source data.}
\label{table:allSrc-super}
\end{table*}


==> tables/office_unsupervised.tex <==
\begin{table*}
  \setlength{\tabcolsep}{4pt}
\centering
                %                 & $A \rightarrow W$  & $D \rightarrow W$  & $W \rightarrow D$  & Average  \\
\begin{tabular}{lcccccc|c}
\toprule
                                 & $A \rightarrow W$  & $A \rightarrow D$ & $D \rightarrow A$& $D \rightarrow W$   & $W \rightarrow A$  &$W \rightarrow D$  & Average  \\
\midrule
%GFK(PLS,PCA)~\cite{gong-cvpr12}   & 15.0 $\pm$ 0.4           & --                       & --                       & 44.6 $\pm$ 0.3           & --                       & 49.7 $\pm$ 0.5           & -- \\
%SA~\cite{sa}                      & 15.3                     & --                       & --                       & 50.1                     & --                       & 56.9                     & -- \\
%DA-NBNN~\cite{da-nbnn}            & 23.3 $\pm$ 2.7           & --                       & --                       & 67.2 $\pm$ 1.9           & --                       & 67.4 $\pm$ 3.0           & -- \\
DLID~\cite{ref:dlid}              & 26.1                     & --                       & --                       & 68.9                     & --                       & 84.9                     & -- \\
DeCAF$_6$ S~\cite{decaf}          & 52.2 $\pm$ 1.7           & --                       & --                       & 91.5 $\pm$ 1.5           & --                       & --                       &  --  \\
DaNN~\cite{da-mmd}                & 35.0 $\pm$ 0.2           & --                       & --                       & 70.5 $\pm$ 0.0           & --                       & 74.3 $\pm$ 0.0           & -- \\
Ganin \etal~\cite{gamin}\footnotemark
	& \textbf{67.3$\pm$ 0.2} & -- & -- & \textbf{94.0$\pm$ 0.1} & -- & {93.7 $\pm$ 0.1} & --\\
Source CNN                  & 56.5 $\pm$ 0.3           & \textbf{64.6 $\pm$ 0.4}  & 47.6 $\pm$ 0.1           & 92.4 $\pm$ 0.3           & 42.7 $\pm$ 0.1           & 93.6 $\pm$ 0.2           & 66.2 \\
\midrule
Ours                              & \textbf{58.0 $\pm$ 0.4}  & 63.4 $\pm$ 0.4           & \textbf{52.4 $\pm$ 0.1}  & \underline{93.8 $\pm$ 0.2}  & \textbf{52.0 $\pm$ 0.1}  & \textbf{96.3 $\pm$ 0.1}  & \textbf{69.3} \\
\bottomrule
\end{tabular}

\caption{Multi-class accuracy evaluation on the standard unsupervised adaptation
  setting with the \emph{Office} dataset.  We evaluate on all 31 categories
  using the standard experimental protocol from \cite{gong-cvpr12}. Here, we
  compare against four state-of-the-art domain adaptation methods as well as a CNN trained on the source data alone.}
\label{table:full-unsuper}
\end{table*}


